Randomized Exploration for Non-Stationary Stochastic Linear Bandits

We investigate two perturbation approaches to overcome conservatism that optimism based algorithms chronically suffer from in practice. The first approach replaces optimism with a simple randomization when using confidence sets. The second one adds random perturbations to its current estimate before maximizing the expected reward. For non-stationary linear bandits, where each action is associated with a $d$-dimensional feature and the unknown parameter is time-varying with total variation $B_T$, we propose two randomized algorithms, Discounted Randomized LinUCB (D-RandLinUCB) and Discounted Linear Thompson Sampling (D-LinTS) via the two perturbation approaches. We highlight the statistical optimality versus computational efficiency trade-off between them in that the former asymptotically achieves the optimal dynamic regret $\tilde{O}(d^{7/8} B_T^{1/4}T^{3/4})$, but the latter is oracle-efficient with an extra logarithmic factor in the number of arms compared to minimax-optimal dynamic regret. In a simulation study, both algorithms show outstanding performance in tackling conservatism issue that Discounted LinUCB struggles with.

==> Stochastic Linear Bandits via Perturbations (1)/macros.tex <==
\newcount\comments  % 0 suppresses notes to selves in text
\comments=1  % TODO: change to 0 for final version
\definecolor{darkgreen}{rgb}{0,0.6,0}
\newcommand{\COMMENT}[2]{\ifnum\comments=1{\color{#1}{#2}}\fi}
\newcommand{\ambuj}[1]{\COMMENT{blue}{[AT: #1]}}
\newcommand{\baekjin}[1]{\COMMENT{red}{[BK: #1]}}
\usepackage{comment} % enables the use of multi-line comments (\ifx \fi) 
\usepackage{url}
\usepackage{algorithm, algorithmicx}
\usepackage{graphicx}
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsmath,amssymb,amsthm}
\usepackage{natbib}
 \usepackage{algpseudocode}
\bibliographystyle{plainnat}

\newtheorem{exercise}{Exercise}
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{example}[theorem]{Example}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}{Assumption}
% \newtheorem*{remark}{Remark}



\newcommnad{\nameA}{\text{Algname}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\Ldim}{\text{Ldim}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}

==> macros.tex <==
\newcount\comments  % 0 suppresses notes to selves in text
\comments=1  % TODO: change to 0 for final version
\definecolor{darkgreen}{rgb}{0,0.6,0}
\newcommand{\COMMENT}[2]{\ifnum\comments=1{\color{#1}{#2}}\fi}
\newcommand{\ambuj}[1]{\COMMENT{blue}{[AT: #1]}}
\newcommand{\baekjin}[1]{\COMMENT{red}{[BK: #1]}}
\usepackage{comment} % enables the use of multi-line comments (\ifx \fi) 
\usepackage{url}
\usepackage{algorithm, algorithmicx}
\usepackage{graphicx}
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsmath,amssymb,amsthm}
\usepackage{natbib}
 \usepackage{algpseudocode}
\bibliographystyle{plainnat}

\newtheorem{exercise}{Exercise}
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{example}[theorem]{Example}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}{Assumption}
% \newtheorem*{remark}{Remark}



\newcommnad{\nameA}{\text{Algname}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\Ldim}{\text{Ldim}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
